A new one point quadrature rule over arbitrary star convex polygon/polyhedron

The Linear Smoothing (LS) scheme \cite{francisa.ortiz-bernardin2017} ameliorates linear and quadratic approximations over convex polytopes by employing a three-point integration scheme. In this work, we propose a linearly consistent one point integration scheme which possesses the properties of the LS scheme with three integration points but requires one third of the integration computational time. The essence of the proposed technique is to approximate the strain by the smoothed nodal derivatives that are determined by the discrete form of the divergence theorem. This is done by the Taylor's expansion of the weak form which facilitates the evaluation of the smoothed nodal derivatives acting as stabilization terms. The smoothed nodal derivatives are evaluated only at the centroid of each integration cell. These integration cells are the simplex subcells (triangle/tetrahedron in two and three dimensions) obtained by subdividing the polytope. The salient feature of the proposed technique is that it requires only $n$ integrations for an $n-$ sided polytope as opposed to $3n$ in~\cite{francisa.ortiz-bernardin2017} and $13n$ integration points in the conventional approach. The convergence properties, the accuracy, and the efficacy of the LS with one point integration scheme are discussed by solving few benchmark problems in elastostatics.

==> newelasintro.tex <==
%\section{Governing equations}
\label{govereqn_weak}

Consider an isotropic linear elastic body that occupies a bounded polynomial domain
$\Omega \subset \Re^d$ which is
bounded by the ($d\!-\!1$)-dimensional surface $\Gamma$ whose
unit outward normal is $\vm{n}$. The boundary is assumed
to admit decompositions $\Gamma=\Gamma_u\cup\Gamma_t$ and
$\emptyset=\Gamma_u\cap\Gamma_t$, where $\Gamma_u$ is the Dirichlet
boundary and $\Gamma_t$ is the Neumann boundary. The closure of
the domain is $\overline{\Omega}\equiv\Omega\cup\Gamma$. Let
$\vm{u} : \Omega \rightarrow \Re^d$ be
the displacement field at a point $\vm{x}$ of the elastic
body when the body is subjected to external tractions
$\bar{\vm{t}}:\Gamma_t\rightarrow \Re^d$ and body forces $\vm{b}:\Omega\rightarrow\Re^d$. The imposed Dirichlet (essential) boundary conditions are
$\hat{\vm{u}}:\Gamma_u\rightarrow \Re^d$. The boundary-value
problem for linear elastostatics is: find
$\vm{u}: \Omega \rightarrow \Re^d$
such that
\begin{subequations}\label{problem:strong_form}
\begin{align}
\quad \bsym{\nabla} \cdot \bsym{\sigma} + \vm{b} &= 0 ~\forall \vm{x} \in \Omega, \\ 
 \quad \vm{u} &= \hat{\vm{u}} ~ \forall \vm{x} \in \Gamma_u, \\
\quad \bsym{\sigma} \cdot \vm{n}
&= \hat{\vm{t}} ~ \forall \vm{x} \in \Gamma_t,
\end{align}
\end{subequations}
where $\bsym{\sigma}$ is the Cauchy stress
tensor. The corresponding weak form is:
find $\vm{u} \in \mathscr{U}$ such that
\begin{subequations}\label{eq:weakform}
\begin{align}
 \quad a(\vm{u},\vm{v})&= \ell(\vm{v}) ~  \forall \vm{v} \in \mathscr{V},\\
a(\vm{u},\vm{v})=\int_{\Omega}\bsym{\sigma}(\vm{u}):\bsym{\varepsilon}(\vm{v})\,\rmd V,\\
\quad
\ell(\vm{v}) = \int_{\Omega}\vm{b}\cdot\vm{v}\,\rmd V + \int_{\Gamma_t}\hat{\vm{t}}\cdot\vm{v}\,\rmd S,
\end{align}
\end{subequations}
where $\bsym{\varepsilon}$ is
the small strain tensor, and $\mathscr{U}$ and $\mathscr{V}$ are the
displacement trial and test spaces:
\begin{subequations}
\begin{align}
\mathscr{U} &:=
\left\{\vm{u}(\vm{x})\in [ C^0(\Omega)]^d : \vm{u} \in
[ \mathcal{W}(\Omega)]^d \subseteq [ H^{1}(\Omega)]^d, \ \vm{u} = \hat{\vm{u}}
\ \textrm{on } \Gamma_u \right\},\nonumber \\
\mathscr{V} &:= \left\{\vm{v}(\vm{x})\in
[ C^0(\Omega) ]^d : \vm{v} \in [ \mathcal{W}(\Omega)]^d \subseteq
[ H^{1}(\Omega) ]^d, \ \vm{v} = \vm{0} \ \textrm{on } \Gamma_u
\right\},\nonumber
\end{align}
\end{subequations}
where the space $\mathcal{W}(\Omega)$ includes linear displacement
fields. The domain is partitioned into elements $\Omega^h$, and on using shape functions $\phi_a$ that span at least the linear space, we substitute vector-valued trial and test functions $\vm{u}^h=\sum_a \phi_a \vm{u}_a$ and $\vm{v}^h=\sum_b \phi_b \vm{v}_b$, respectively, into~\eref{eq:weakform} and apply a standard Galerkin procedure to obtain the discrete weak form: find $\vm{u}^h \in \mathscr{U}^h$ such that
\begin{equation}\label{eq:discweakform}
 \quad a(\vm{u}^h,\vm{v}^h)= \ell(\vm{v}^h) ~ \forall \vm{v}^h \in \mathscr{V}^h,
\end{equation}
which leads to the following system of linear equations:
\begin{subequations}\label{eq:weakform_disc}
\begin{align}
\mat{K}\mat{u}&=\mat{f},\\
\mat{K}=\sum_h \mat{K}^h &=\sum_h\int_{\Omega^h}\mat{B}^\transpose\mat{C}\mat{B}\,\rmd V,\\
\mat{f} = \sum_h \mat{f}^h &=\sum_h\left(\int_{\Omega^h}\mat{N}^\transpose\vm{b}\,\rmd V + \int_{\Gamma_t^h}\mat{N}^\transpose\hat{\vm{t}}\,\rmd S\right),
\end{align}
\end{subequations}
where $\mat{K}$ is the assembled stiffness matrix, $\mat{f}$ the assembled nodal force vector, $\mat{u}$ the assembled vector of nodal displacements, $\mat{N}$ is the matrix of shape functions,
$\mat{C}$ is the constitutive matrix for an isotropic linear elastic
material, and $\mat{B}=\bsym{\nabla}_s\mat{N}$ is the strain-displacement matrix that is computed using the derivatives of the shape functions.

The shape functions over arbitrary polygons/polyhedra are collectively called as `barycentric coordinates'. Because there is no unique way to represent the shape functions over polytopes, there are multiple approaches to construct them. Interested readers are referred to Reference~\cite{Sukumar2006} for a detailed discussion on the construction of shape functions over polytopes. In this paper, Wachspress interpolants are used.

The main issue in computing the stiffness matrix defined in~\eref{eq:weakform_disc} for polygonal/polyhedral elements is the construction of sufficiently accurate integration rules. In an effort to improve the accuracy, a modified version of the strain-displacement matrix is usually defined to compute the stiffness matrix. This modified strain-displacement matrix is denoted by $\tilde{\mat{B}}$ and is constructed using smoothing domains. A smoothing technique that yields linear strains and improved accuracy in polygonal/polyhedral finite elements is proposed in this paper. Thus,the stiffness matrix is computed as for the constant smoothing:
\begin{equation}\label{eq:modstiffness}
\mat{\tilde{K}}=\sum_h \mat{\tilde{K}}^h=\sum_h\int_{\Omega^h}\tilde{\mat{B}}^\transpose\mat{C}\tilde{\mat{B}}\,\rmd V,
\end{equation}
\textcolor{red}{This is also true for linear smoothing technique, where only the matrix $\tilde{\mat{B}}$ varies, with a linear smoothed strain-displacement operator (see Section 4.2) as opposed to a constant smoothed strain-displacement operator (see Section 4.1)~\cite{liudai2007,natarajanbordas2015}.}

==> onePtQuad.tex <==
The next step in the process is to compute the modified strain-displacement matrix to build the stiffness matrix~\eref{eq:modstiffness}. To this end we rely on the smoothed finite element method (SFEM), which has its origin in the stabilized conforming nodal integration (SCNI)~\cite{chen:2001:ASC} for meshfree methods, where the strain field is sampled at the nodes by smoothing the nodal strain on the boundary of a representative nodal volume (`the smoothed domain'). In particular, we focus our attention on the cell-based smoothing technique. In the CSFEM, the elements are divided into subcells as shown in~\fref{fig:subcellRepre}. In this paper, we use triangles in two dimensions and tetrahedra in three dimensions. The strain smoothing technique is then applied within each subcell to evaluate the modified strain. For simplicity of the notation, the derivation of the smoothing scheme is given in detail only for two-dimensions. The Cartesian coordinate system is chosen, where for convenience $x\equiv x_1$ and $y\equiv x_2$. In addition, $n_j$ ($j=1,2$) is the $j$-th component of the unit outward normal to a cell edge in the Cartesian coordinate system. The discrete strain field $\tilde{\varepsilon }_{ij}^h$ that yields the modified strain-displacement matrix $\tilde{\mat{B}}$ that is used to build the stiffness matrix is computed by a weighted average of the standard strain field $ {\varepsilon }_{ij}^h$ in each subcell $\Omega_C^h$, as follows:
\begin{equation}
\tilde {\varepsilon }_{ij}^h (\xx)=\int_{\Omega_C^h}
{\varepsilon _{ij}^h (\xx) f(\xx) \rmd V },
\label{eqn:epsilonvar}
\end{equation}
where $f$ is a smoothing function. On writing~\eref{eqn:epsilonvar} at the basis functions derivatives level, its right-hand side can be expressed in terms of the divergence theorem, as follows:
\begin{equation}\label{eq:divconsistency}
\int_{\Omega_C^h}\phi_{a,j}f(\vm{x})\, \rmd V  =  \int_{\Gamma_C^h}\phi_a f(\vm{x})n_j\, \rmd S - \int_{\Omega_C^h}\phi_a f_{,j}(\vm{x})\, \rmd V.
\end{equation}
\eref{eq:divconsistency} was coined as \textit{divergence consistency} in Duan et al.~\cite{duan:2012:SOI,duan:2014:CEF,duan:2014:FPI}, where it was introduced to correct integration errors in second- and third-order meshfree approximations. This divergence consistency was later used by Sukumar to correct integration errors in quadratic maximum-entropy serendipity polygonal elements~\cite{Sukumar2013} and by Ortiz-Bernardin and co-workers to correct integration errors in the volume-averaged nodal projection (\texttt{VANP}) meshfree method~\cite{ortiz:VAN:2015,ortiz:IRN:2015}.

\begin{figure}[htpb]
\centering
\begin{subfigure}
		\centering
\includegraphics[width=0.3\textwidth]{./Figures/subcell.eps}
\caption*{(a) Discertization of arbitrary polygon into triangular subcell using virtual point shown by 'open' circle.}	
	\end{subfigure}
	\quad
	\begin{subfigure}
		\centering
\includegraphics[width=0.3\textwidth]{./Figures/subcellwithpoint.eps}
\caption*{(b) Number of integration point used per subcell}
	\end{subfigure}\caption{Schematic representation of the one point integration technique. The nodes are depicted by the filled circles, while the Gauss point per edge is shown by filled squares. The smoothed derivatives are computed at the 'open' squares. }
\label{fig:subcellRepre}
\end{figure}

The orthogonality condition between the compatible and the smoothed nodal derivatives at the point of integration to be satisfied is given as;

\begin{equation}
\int\limits_{\Omega_L} \textbf{q}(\textbf{x})\left(\phi}_{I,x} - \tilde{\phi}_{I,x} \right)~\mathrm{d}\Omega
\end{equation}


To introduce the high order derivatives into \eref{eq:modstiffness}, Taylor expansion of $\tilde{\phi}_{I,x},(\xx)~\bq(\xx)$ and $\phi_I(\xx)$ is used:
\begin{align}
\begin{split}
\tilde{\phi}_{I,x}(\xx)  &= \tilde{\phi}_{I,x}(\xx_c) + (x-x_c) \tilde{\phi}_{I,xx}(\xx_c) + (y-y_c)\tilde{\phi}_{I,xy}(\xx_c) + \mathcal{O}( (\xx-\xx_c)^2) \\
\bq(\xx) &= \bq(\xx_c) + (x-x_c) \bq_{,x}(\xx) + (y-y_c)\bq_{,y}(\xx) \\
\phi_{I}(\xx)  &= \phi_{I}(\xx_c) + (x-x_c) \phi_{I,x}(\xx_c) + (y-y_c)\phi_{I,y},(\xx_c) + \frac{1}{2} (x-x_c)^2 \phi_{I,xx}(\xx_c)  \\  &+  (x-x_c)(y-y_c)\phi_{I,xy}(\xx_c) + \frac{1}{2} (y-y_c)^2 \phi_{I,yy}(\xx_c) + \mathcal{O}( (\xx-\xx_c)^3)
\end{split}
\label{eq:taylorexpansion}
\end{align}
where $\xx_c = \left\{x_c,y_c\right\}$ is the center of the cell. Upon substituting \eref{eq:taylorexpansion} into \eref{eq:divconsistency}, we have:
\begin{equation}
\begin{split}
\bq(\xx_c)A\tilde{\phi}_{I,x}(\xx_c) + \left[ \bq_x(\xx_c) I_c^{xx} + \bq_y(\xx_c) I_c^{xy} \right] \tilde{\phi}_{I,xx}(\xx_c) + \left[ \bq_{,x}(\xx_c) I_c^{xy} + \bq_{,y}(\xx_c)I_c^{yy} \right] \tilde{\phi}_{I,xy}(\xx_c) \\ = \int\limits_\Gamma \phi_I(\xx) \bq(\xx) \mathbf{n}~\mathrm{d}\Gamma - \left[ A\phi_I(\xx_c) + \frac{1}{2}I_c^{xx} \phi_{I,xx}(\xx_c) + I_c^{xy}\phi_{I,xy}(\xx_c) + \frac{1}{2} I_c^{yy} \phi_{I,yy}(\xx_c) \right]
\end{split}
\label{eq:newtaylorform}
\end{equation}
where $A = \int\limits_\Omega \mathrm{d}\Omega$ is the area of the integration domain $\Omega$, the first order area moments with respect to cell center $\xx_c$ vanish and the second order area moments are given by: 
\begin{equation}
\left\{ \begin{array}{c} I_c^{xx} \\ I_c^{xy} \\ I_c^{yy} \end{array} \right\} = \int\limits_\Omega \left\{ \begin{array}{c} (x-x_c)^2 \\ (x-x_c)(y-y_c) \\ (y-y_c)^2 \end{array} \right\}~\mathrm{d}\Omega
\end{equation}
\begin{remark}
For a regular polygon, the second order area moment $I_c^{xy}$ also vanish apart from the first order area moments.
\end{remark}
For $\bq(\xx) = \left[ \begin{array}{ccc} 1 & x & y \end{array} \right]$ and using numerical integration to evaluate the boundary integral, \eref{eq:newtaylorform} leads to the following system of linear equations:
\begin{equation}
\mat{W} \mat{d}_j = \mat{f}_j, \quad j = 1,2
\label{eq:lineareqn}
\end{equation}
where,
\begin{subequations}
\begin{align}
\mat{W} &= \left[ \begin{array}{ccc} A & 0 & 0 \\ Ax_c & I_c^{xx} & I_c^{xy} \\ Ay_c & I_c^{xy} & I_c^{yy} \end{array} \right] \\
\mat{f}_1 &= \left\{ \begin{array}{c} \sum\limits_{L=1}^3 \sum\limits_{G=1}^2 \phi_I(\xx_G)n_x^Lw_G \\ \sum\limits_{G=1}^2 \phi_I(\xx_G)x_G n_x^Lw_G - Fg \\ \sum\limits_{G=1}^2 \phi_I(\xx_G) y_G n_x^Lw_G \end{array} \right\} \\
\mat{f}_2 & = \left\{ \begin{array}{c} \sum\limits_{L=1}^3 \sum\limits_{G=1}^2 \phi_I(\xx_G)n_x^Lw_G \\ \sum\limits_{G=1}^2 \phi_I(\xx_G)x_G n_x^Lw_G \\ \sum\limits_{G=1}^2 \phi_I(\xx_G) y_G n_x^Lw_G - Fg \end{array} \right\}
\end{align}
\end{subequations}
where $Fg = A\phi_I(\xx_c) + \frac{1}{2}I_c^{xx}\phi_{I,xx}(\xx_c) + I_c^{xy} \phi_{I,xy}(\xx_c) + \frac{1}{2} I_c^{yy} \phi_{I,yy}(\xx_c)$ and $\phi_I(\xx_c),\, \phi_{I,xx}(\xx_c) \, \phi_{I,yy}(\xx_c)$ and $\phi_{I,xy}(\xx_c)$ are the barycentric coordinates and its derivatives evaluated at the center of the cell. The solution vector is given by:
\begin{subequations}
\begin{align}
\mat{d}_1 &= \left\{ \begin{array}{c} \tilde{\phi}_{I,x}(\xx_c) \\ \tilde{\phi}_{I,xx}(\xx_c) \\ \tilde{\phi}_{I,xy}(\xx_c) \end{array} \right\} \\
\mat{d}_2 &= \left\{ \begin{array}{c} \tilde{\phi}_{I,y}(\xx_c) \\ \tilde{\phi}_{I,yx}(\xx_c) \\ \tilde{\phi}_{I,yy}(\xx_c) \end{array} \right\}
\end{align}
\end{subequations}
\begin{remark}
\eref{eq:lineareqn} always have an unique solution provided the triangles do not degenerate to a line.
\end{remark}

==> oneptquadnew.tex <==
The next step in the process is to compute the modified strain-displacement matrix to build the stiffness matrix~\eref{eq:modstiffness}. To this end we rely on the smoothed finite element method (SFEM), which has its origin in the stabilized conforming nodal integration (SCNI)~\cite{chen:2001:ASC} for meshfree methods, where the strain field is sampled at the nodes by smoothing the nodal strain on the boundary of a representative nodal volume (`the smoothed domain'). In particular, we focus our attention on the cell-based smoothing technique. In the CSFEM, the elements are divided into subcells as shown in~\fref{fig:subcellRepre}. In this paper, we use triangles in two dimensions and tetrahedra in three dimensions. The strain smoothing technique is then applied within each subcell to evaluate the modified strain. For simplicity of the notation, the derivation of the smoothing scheme is given in detail only for two-dimensions. The Cartesian coordinate system is chosen, where for convenience $x\equiv x_1$ and $y\equiv x_2$. In addition, $n_j$ ($j=1,2$) is the $j$-th component of the unit outward normal to a cell edge in the Cartesian coordinate system. The discrete strain field $\tilde{\varepsilon }_{ij}^h$ that yields the modified strain-displacement matrix $\tilde{\mat{B}}$ that is used to build the stiffness matrix is computed by a weighted average of the standard strain field $ {\varepsilon }_{ij}^h$ in each subcell $\Omega_C^h$, as follows:
\begin{equation}
\tilde {\varepsilon }_{ij}^h (\xx)=\int_{\Omega_C^h}
{\varepsilon _{ij}^h (\xx) f(\xx) \rmd V },
\label{eqn:epsilonvar}
\end{equation}
where $f$ is a smoothing function. On writing~\eref{eqn:epsilonvar} at the basis functions derivatives level, its right-hand side can be expressed in terms of the divergence theorem, as follows:
\begin{equation}\label{eq:divconsistency}
\int_{\Omega_C^h}\phi_{a,j}f(\vm{x})\, \rmd V  =  \int_{\Gamma_C^h}\phi_a f(\vm{x})n_j\, \rmd S - \int_{\Omega_C^h}\phi_a f_{,j}(\vm{x})\, \rmd V.
\end{equation}
\eref{eq:divconsistency} was coined as \textit{divergence consistency} in Duan et al.~\cite{duan:2012:SOI,duan:2014:CEF,duan:2014:FPI}, where it was introduced to correct integration errors in second- and third-order meshfree approximations. This divergence consistency was later used by Sukumar to correct integration errors in quadratic maximum-entropy serendipity polygonal elements~\cite{Sukumar2013} and by Ortiz-Bernardin and co-workers to correct integration errors in the volume-averaged nodal projection (\texttt{VANP}) meshfree method~\cite{ortiz:VAN:2015,ortiz:IRN:2015}.

\begin{figure}[htpb]
\centering
\begin{subfigure}
		\centering
\includegraphics[width=0.3\textwidth]{./Figures/subcell.eps}
\caption*{(a) Discertization of arbitrary polygon into triangular subcell using virtual point shown by 'open' circle.}	
	\end{subfigure}
	\quad
	\begin{subfigure}
		\centering
\includegraphics[width=0.3\textwidth]{./Figures/subcellwithpoint.eps}
\caption*{(b) Number of integration point used per subcell}
	\end{subfigure}\caption{Schematic representation of the one point integration technique. The nodes are depicted by the filled circles, while the Gauss point per edge is shown by filled squares. The smoothed derivatives are computed at the 'open' squares. }
\label{fig:subcellRepre}
\end{figure}

The orthogonality condition between the compatible and the smoothed nodal derivatives at the point of integration to be satisfied is given as;
\begin{equation}
\int\limits_{\Omega_L} f(\xx)\left(\phi_{I,x} - \tilde{\phi}_{I,x} \right)~\mathrm{d}\Omega =0
\label{Oc}
\end{equation}
The above Equation \eref{Oc} can be rewritten as;

\begin{equation}
\int\limits_{\Omega_L} \tilde{\phi}_{I,x} ~ f(\xx)~ \mathrm{d}\Omega = \int\limits_{\Omega_L} \phi_{I,x} ~ f(\xx)~ \mathrm{d}\Omega
\end{equation}

Using Gauss divergence theorem. We get;

\begin{equation}
\int\limits_{\Omega_L} \tilde{\phi}_{I,x} ~ f(\xx)~ \mathrm{d}\Omega = \int\limits_{\Gamma_L} \phi_I ~f(\xx)~ n_{i}~ \mathrm{d} \Gamma - \int\limits_{\Omega_L} \phi_I~ f_{,j}(\vm{x}) ~ \mathrm{d}\Omega
\label{dc}
\end{equation} 
The above Equation \eref{dc} is used to evaluated the modified derivatives. For $f(\xx) =[1]$ is used in SFEM \cite{liudai2007} which is only consistent for linear approximation. Futhermore, if $f(\xx) = [1~ x ~y]$ which is the key feature in the formulation of linear smoothing technique presented in our previous paper \cite{NME:NME5324}, which allows to be consistent in higher order approximation. In order to do we use 3\textit{n} integration points where \textit{n} is the number of edges of the arbitrary polygon. So, in order to minimize the quadrature for numerical integration we are presenting one point integration scheme for the same $f(\xx)$ over the smoothing domain. This is done by using Taylor's expansion of the week form and using the smoothed higher order derivatives in the week form.

To introduce the high order derivatives into \eref{eq:modstiffness}, Taylor expansion of $\tilde{\phi}_{I,x},(\xx)~\bq(\xx)$ and $\phi_I(\xx)$ is used:
\begin{align}
\begin{split}
\tilde{\phi}_{I,x}(\xx)  &= \tilde{\phi}_{I,x}(\xx_c) + (x-x_c) \tilde{\phi}_{I,xx}(\xx_c) + (y-y_c)\tilde{\phi}_{I,xy}(\xx_c) + \mathcal{O}( (\xx-\xx_c)^2) \\
\bq(\xx) &= \bq(\xx_c) + (x-x_c) \bq_{,x}(\xx) + (y-y_c)\bq_{,y}(\xx) \\
\phi_{I}(\xx)  &= \phi_{I}(\xx_c) + (x-x_c) \phi_{I,x}(\xx_c) + (y-y_c)\phi_{I,y},(\xx_c) + \frac{1}{2} (x-x_c)^2 \phi_{I,xx}(\xx_c)  \\  &+  (x-x_c)(y-y_c)\phi_{I,xy}(\xx_c) + \frac{1}{2} (y-y_c)^2 \phi_{I,yy}(\xx_c) + \mathcal{O}( (\xx-\xx_c)^3)
\end{split}
\label{eq:taylorexpansion}
\end{align}
where $\xx_c = \left\{x_c,y_c\right\}$ is the center of the cell. Upon substituting \eref{eq:taylorexpansion} into \eref{eq:divconsistency}, we have:
\begin{equation}
\begin{split}
\bq(\xx_c)A\tilde{\phi}_{I,x}(\xx_c) + \left[ \bq_x(\xx_c) I_c^{xx} + \bq_y(\xx_c) I_c^{xy} \right] \tilde{\phi}_{I,xx}(\xx_c) + \left[ \bq_{,x}(\xx_c) I_c^{xy} + \bq_{,y}(\xx_c)I_c^{yy} \right] \tilde{\phi}_{I,xy}(\xx_c) \\ = \int\limits_\Gamma \phi_I(\xx) \bq(\xx) \mathbf{n}~\mathrm{d}\Gamma - \left[ A\phi_I(\xx_c) + \frac{1}{2}I_c^{xx} \phi_{I,xx}(\xx_c) + I_c^{xy}\phi_{I,xy}(\xx_c) + \frac{1}{2} I_c^{yy} \phi_{I,yy}(\xx_c) \right]
\end{split}
\label{eq:newtaylorform}
\end{equation}
where $A = \int\limits_\Omega \mathrm{d}\Omega$ is the area of the integration domain $\Omega$, the first order area moments with respect to cell center $\xx_c$ vanish and the second order area moments are given by: 
\begin{equation}
\left\{ \begin{array}{c} I_c^{xx} \\ I_c^{xy} \\ I_c^{yy} \end{array} \right\} = \int\limits_\Omega \left\{ \begin{array}{c} (x-x_c)^2 \\ (x-x_c)(y-y_c) \\ (y-y_c)^2 \end{array} \right\}~\mathrm{d}\Omega
\end{equation}
\begin{remark}
For a regular polygon, the second order area moment $I_c^{xy}$ also vanish apart from the first order area moments.
\end{remark}
For $\bq(\xx) = \left[ \begin{array}{ccc} 1 & x & y \end{array} \right]$ and using numerical integration to evaluate the boundary integral, \eref{eq:newtaylorform} leads to the following system of linear equations:
\begin{equation}
\mat{W} \mat{d}_j = \mat{f}_j, \quad j = 1,2
\label{eq:lineareqn}
\end{equation}
where,
\begin{subequations}
\begin{align}
\mat{W} &= \left[ \begin{array}{ccc} A & 0 & 0 \\ Ax_c & I_c^{xx} & I_c^{xy} \\ Ay_c & I_c^{xy} & I_c^{yy} \end{array} \right] \\
\mat{f}_1 &= \left\{ \begin{array}{c} \sum\limits_{L=1}^3 \sum\limits_{G=1}^2 \phi_I(\xx_G)n_x^Lw_G \\ \sum\limits_{G=1}^2 \phi_I(\xx_G)x_G n_x^Lw_G - Fg \\ \sum\limits_{G=1}^2 \phi_I(\xx_G) y_G n_x^Lw_G \end{array} \right\} \\
\mat{f}_2 & = \left\{ \begin{array}{c} \sum\limits_{L=1}^3 \sum\limits_{G=1}^2 \phi_I(\xx_G)n_x^Lw_G \\ \sum\limits_{G=1}^2 \phi_I(\xx_G)x_G n_x^Lw_G \\ \sum\limits_{G=1}^2 \phi_I(\xx_G) y_G n_x^Lw_G - Fg \end{array} \right\}
\end{align}
\end{subequations}
where $Fg = A\phi_I(\xx_c) + \frac{1}{2}I_c^{xx}\phi_{I,xx}(\xx_c) + I_c^{xy} \phi_{I,xy}(\xx_c) + \frac{1}{2} I_c^{yy} \phi_{I,yy}(\xx_c)$ and $\phi_I(\xx_c),\, \phi_{I,xx}(\xx_c) \, \phi_{I,yy}(\xx_c)$ and $\phi_{I,xy}(\xx_c)$ are the barycentric coordinates and its derivatives evaluated at the center of the cell. The solution vector is given by:
\begin{subequations}
\begin{align}
\mat{d}_1 &= \left\{ \begin{array}{c} \tilde{\phi}_{I,x}(\xx_c) \\ \tilde{\phi}_{I,xx}(\xx_c) \\ \tilde{\phi}_{I,xy}(\xx_c) \end{array} \right\} \\
\mat{d}_2 &= \left\{ \begin{array}{c} \tilde{\phi}_{I,y}(\xx_c) \\ \tilde{\phi}_{I,yx}(\xx_c) \\ \tilde{\phi}_{I,yy}(\xx_c) \end{array} \right\}
\end{align}
\end{subequations}
\begin{remark}
\eref{eq:lineareqn} always have an unique solution provided the triangles do not degenerate to a line.
\end{remark}
